Improving Upon the generalized c-mu rule: a Whittle approach

Scheduling a stream of jobs whose holding cost changes over time is a classic and practical problem. Specifically, each job is associated with a holding cost (penalty), where a job's instantaneous holding cost is some increasing function of its class and current age (the time it has spent in the system since its arrival). The goal is to schedule the jobs to minimize the time-average total holding cost across all jobs. The seminal paper on this problem, by Van Mieghem in 1995, introduced the generalized c-mu rule for scheduling jobs. Since then, this problem has attracted significant interest but remains challenging due to the absence of a finite-dimensional state space formulation. Consequently, subsequent works focus on more tractable versions of this problem. This paper returns to the original problem, deriving a heuristic that empirically improves upon the generalized c-mu rule and all existing heuristics. Our approach is to first translate the holding cost minimization problem to a novel Restless Multi-Armed Bandit (R-MAB) problem with a finite number of arms. Based on our R-MAB, we derive a novel Whittle Index policy, which is both elegant and intuitive.

==> related.tex <==
\section{Related Works}
\label{sec:related}
\textbf{The $c\mu$ rule and the generalized $c\mu$ rule}  
% \mor{In reading this section, it is not clear to me whether you're assuming that job sizes are exponentially distributed or generally distributed.  You should state it.  Assuming general service time, the average processing time is not the same as the average remaining processing time.}
The main solution found in the operations literature for the scheduling problem of minimizing time-average total holding cost is the $c\mu$ rule, which is introduced by Cox and Smith in 1961 (\cite{cox2020queues}). The $c\mu$ rule is as follows. Suppose jobs of class $k$ have average processing time $1/\mu_k$ \mor{Do you want to instead talk about failure rate here, so this applies to the general setting, which is coming up in the next paragraph?} and accrue a holding cost of $c_k$ for every time unit they spend in system. With each class $k$, we associate the index $c_k\mu_k$. We serve the job with highest priority index at each decision point. The $c\mu$ rule is known to be optimal for scheduling multi-class M/M/1 queues (where the job sizes are exponentially distributed) with fixed holding costs~\cite{cox2020queues}. 

Various attempts have been made to generalize the $c\mu$ rule over the years. One of the most important works is Van Mieghem's paper from 1995 \cite{van1995dynamic}.  Van Mieghem considered the setting where the (accumulated) holding cost is a convex function of each job's delay,  and proposed the 
 \enquote{generalized} $c\mu$ rule which indexes jobs by the product of their instantaneous holding cost and instantaneous service rate.  This policy was shown to be asymptotically optimal in the diffusion limit (i.e. both arrival and service rates scale to infinity and the total traffic goes to 1) for multi-class M/G/1 queues with convex accumulated holding cost~\cite[Proposition 8]{van1995dynamic}. There are other works further proving asymptotic optimality of the generalized $c\mu$ rule (or its analogue) in many other settings such as multiple servers and system with abandonment (\cite{mandelbaum2004scheduling,atar2010cmu,  long2020dynamic}), but all these optimality results rely on the diffusion limit.
 % \mor{These references are all on the generalized $c \mu$ rule, right?  Also a reminder to me to discuss the diffusion limit.} 

 However, although the generalized $c\mu$ rule is optimal under the diffusion limit, it is known to be suboptimal under the normal traffic regime, and there is a need for policies beyond the generalized $c\mu$ rule. There are many works on scheduling convex  holding cost (e.g., \cite{gurvich2009scheduling, atar2004scheduling,bispo2013single,larrnaaga2016dynamic}), but all these papers are in the {\em queue-length holding cost setting}, where the holding cost of each class is viewed as a function of the number of jobs in the class at that time. That is, the holding cost of class $i$ increases as a convex function of the number of jobs of class $i$. Clearly, this setting is quite different from our setting where the holding cost is a function of each job's age, which is the original setting raised in \cite{van1995dynamic}. The queue-length holding cost setting is complementary to our approach, but the policies in each setting cannot be directly transferred to the other.
 
 
 % For example, it is shown that the optimal scheduling policy should take the ``load'' of each class into consideration (\cite{bispo2013single}), which does not appear in the generalized c$\mu$ rule. Thus there is a need for other policies. 

 \textbf{The Whittle Index approach}
The Whittle Index approach was first raised by Whittle in 1988 to develop a heuristic for the restless bandit problem (\cite{whittle1988restless}). The idea is to relax the hard constraint that only one arm can be pulled at a time to a time-average constraint, thus utilizing the Lagrange multiplier to solve the relaxed problem. There are recent works proving asymptotic optimality of the Whittle Index (e.g., \cite{ayesta2021computation}), and the Whittle Index has also long been shown to be a surprisingly good heuristic (see \cite{nino2007dynamic} for a discussion). See \cite{nino2023markovian} for a recent review.
 
There is a subset of the Whittle Index scheduling looking at the problem of minimizing mean holding cost for nonconstant holding cost functions~\cite{ansell2003whittle, larranaga2014index, glazebrook2003index}. However, these papers adopt the  queue-length holding cost setting, which naturally leads to a discrete-state Markov chain, enabling  analysis. By contrast, in our setting, converting the scheduling problem into a continuous Markov chain is non-trivial. 

% However, when the holding cost is a function of the number of jobs in the class, there is an immediate discrete-state Markov chains that can be analyzed using Whittle's Index approach. In our problem where the holding cost is a function of delay, we need to first construct a (continuous) Markov chain (bandit), thus it is more difficult.

The Whittle Index has also been applied to our age-based holding cost setting \cite{anand2018whittle,aalto2024whittle}. However, both of these papers considered a static version of the problem, where all jobs are present at time $0$ and there are no new arrivals; thus, these papers are also quite different from our work. One drawback of these heuristics, which are derived from the static version settings, is that they do not incorporate the arrival rate (and consequently the load) of each class into their index, which is suggested to be necessary in \cite{bispo2013single}. Both papers~\cite{anand2018whittle,aalto2024whittle} note the analytical intractability of not only the open dynamic delay-based holding cost minimization MAB problem, but even its single arm relaxed Whittle formulation. Our result derives an optimal solution to this single arm relaxation in the M/M/1 setting. Also, in Section \ref{sec:simulation}, we show that our policy outperforms the heuristic in \cite{aalto2024whittle}.
\mor{Does this mean we also outperform \cite{anand2018whittle}?}
\zl{\cite{anand2018whittle} is a special case of \cite{aalto2024whittle}, and their heuristic does not apply to our setting.}

% A very recent work \cite{aalto2024whittle} also uses Whittle's Index in the time-convex... but closed system. The result is more general (IHR job size instead of exponential), but independent of the load. 

% Notably, all of those Whittle's Index policies are just heuristics and the performance is evaluated through simulations. However, in this paper, we also prove our policies' optimality in a special case, which is also a difference from the literature.

% 
